INVARLLM: LLM-assisted Physical Invariant Extraction for Cyber-Physical Systems Anomaly Detection

Cyber-Physical Systems (CPS) are vulnerable to cyber-physical attacks that violate physical laws. While invariant-based anomaly detection is effective, existing methods are limited: data-driven approaches lack semantic context, and physics-based models require extensive manual work. We propose INVARLLM, a hybrid framework that uses large language models (LLMs) to extract semantic information from CPS documentation and generate physical invariants, then validates these against real system data using a PCMCI+-inspired K-means method. This approach combines LLM semantic understanding with empirical validation to ensure both interpretability and reliability. We evaluate INVARLLM on SWaT and WADI datasets, achieving 100% precision in anomaly detection with no false alarms, outperforming all existing methods. Our results demonstrate that integrating LLM-derived semantics with statistical validation provides a scalable and dependable solution for CPS security.

==> note.tex <==
Highlights:

1. LLM is able to extract information from cps documents

1.1 illustrate what is illustrated in the cps documents
    1.1.1 procedure descriptions and separations
    1.1.2 tables of data points
    1.1.3 diagrams showing the topology of devices
    1.1.4 description of control procedures

1.2 discuss different strategies
    1.2.1 document parsing
    1.2.2 embedding vs non-embedding
    1.2.3 different llms (reasoning vs non-reasoning)
    1.2.4 prompt organization
    1.2.5 when to stop 

2 combination of data-based approach and semantic
    2.1 different approaches
        2.1.1 data to llm directly
        2.1.2 llm plus statistic results
        2.1.3 llm for hypothetical and stat for validation
        
    2.2 invariant validation
        2.2.1 PCMCI searching
            more efficient for complex relationship
            \textbf{node embedding}
            
        2.2.2 validation dataset
            validating the accepted invariants on the training dataset, for reducing false alarms

    2.3 anomaly detection 
        insight: \textbf{sliding window change}
        


3. Semantic information is helpful for generating more comprehensive invariants

    3.1 limitations of statistical algorithms (without considering semantics)
    False Negatives

    3.2 limitations of semantic-only solutions
    False Positives


==> sections/archive.tex <==



; 2) \textbf{Invariants Verification Phase}, which validates the hypothetical invariants generated in the first phase using training datasets to exclude those deviating from the ground truth; 3) \textbf{Anomaly Detection Phase}, which applies the verified invariants to real-time data streams from the CPS deployment and reports data points that violate these invariants as anomalies.\\
\noindent\textbf{Challenges:} While seemingly promising, there are several prominent challenges in the design and implementation of each phase. 1) There are no regulated formats for CPS documentation, allowing CPS developers to illustrate their designs using various formats such as text descriptions, tables, and diagrams. Without accurately parsing information in these diverse formats, the LLM may not be able to answer questions using the most relevant information. 2) LLMs are well-known to suffer from the issue of hallucination, where LLMs may include fabricated content in the response that is not reasonable and explainable. 3), multiple parameters are involved in the invariants validation and anomaly detection phases, which can significantly affect the performance of the detection results. Identifying a set of parameters that achieve optimal detection performance is a non-trivial task. 4) Although physical invariants are governed by inherent physical laws and procedures, they may also suffer from drifting over time. Constant invariants for anomaly detection will gradually become outdated, deviating from the physical ground truth, and producing more false alarms.
To demonstrate the versatility and robustness of our approach, we apply it to two distinct real-world public CPS datasets: the Secure Water Treatment (SWaT) dataset\cite{b39,b40} and the HAI dataset\cite{b28}. as described in the Introduction, to illustrate the workflow.\\

In the first phase, LLMs infer possible physical invariants based on testbed specification documents provided by CPS developers. For example, the HAI testbed includes four major physical processes: Boiler Process, Turbine Process, Water-treatment Process, and Hardware-in-the-loop Simulator. The developers clearly define the functions, specifications, and connections of hardware components in the first three processes. We augment the large language model into an intelligent agent comprising modules for document parsing, retrieval-augmented generation (RAG), and chain-of-thought prompts (CoT). The agent takes the PDF files of testbed specifications as input and automatically produces a list of possible physical invariants with detailed explanations for each. As illustrated in Figure~\ref{fig:overview}
, the LLM successfully identifies a physical invariant concerning "water mass balance," which elucidates that the water level (LIT01) is determined by the equilibrium between the inflow rate, controlled by LCV01D, and the outflow rate, modulated by FCV03D. Thus, the rate of change in water level at any given moment is inferable from the positions of the two water valves. The agent further formulates the invariant into the equation $\frac{d}{dt}LIT01(t) = C_{1} \cdot LCV01D(t) + C_{2} \cdot FCV03D(t)$. The undetermined coefficients can be derived using regression with training data points.
% \begin{equation}\label{equ:lc-example}
%     \frac{d(LIT01)}{d(t)} = \alpha*(LCV01D) + \beta*(FCV03D)
% \end{equation}
In the second phase, we validate the correctness of each hypothetical physical invariant generated in the first phase. Our insight is that a physical invariant if it exists, will remain stable during the data collection period. Specifically, the coefficients in the invariant equations should remain constant when derived using different segments of the training dataset. If the learned pattern changes over short periods, it could result in a high number of false alarms when used for detecting anomalies. To validate hypothetical invariants, we conduct multi-fold cross-validation on the training dataset. We split the dataset into $K$ bins, derive the coefficients from each bin, and apply them to the other bins. A hypothetical invariant is accepted only if the patterns match across all bins. As shown in Figure~\ref{fig:overview}
, the values of $C_{1}$ and $C_{2}$ remain constant in the training dataset, which validates the physical invariant.
Finally, in the third phase, we apply the validated physical invariants to detect anomalous data points in the testing dataset. In the example, the validated physical invariant $
\frac{d}{dt}LIT01(t) = C_{1} \cdot LCV01D(t) - C_{2} \cdot FCV03D(t) $ is applied to the testing dataset using the same approach as in the invariant validation step. However, the validation is conducted in small sliding windows instead of cross-validation, as testing data is gradually accumulated in real-world deployments. Regression is performed in each sliding window to obtain the sequence of values for $C_{1}$ and $C_{2}$. Data points that fall outside the threshold are detected as anomalies. In the example, an abnormally low $\beta$ value is observed when the attack scenario \verb|AP15| is launched due to the fake readings from the water level sensor LIT01.
In the remainder of this section, we will illustrate the details of AnomalyLLM's design, particularly focusing on how it addresses the aforementioned challenges.




% we extract the HAI CPS testbed specification documents are utilized as the contextual input to extract potential physical invariants by harnessing the capabilities of LLMs. Specifically, we convert the PDF file of the testbed specification into textual segments, tables, and figures, subsequently embedding these elements into a multi-modal knowledge vector store. This process is facilitated by a multi-modal Retrieval-Augmented Generation (RAG) application that utilizes the vector store as its contextual foundation. We formulate a chain-of-thought prompt designed to elicit the generation of hypothetical physical invariants derived from the documentation by the LLM. 



% \noindent\textbf{Physical Invariants Extraction}
% In the initial phase, 


% \noindent\textbf{Physical Invariants Validation}
% The hypothetical physical invariants identified in the previous step are inferred by LLMs based on their extensive knowledge base and may not align with empirical physical realities. Therefore, this subsequent step involves the validation of these invariants by using the training dataset to eliminate those hypothetical invariants that are implausible, thereby preventing the generation of false alarms. The validation is performed by doing liner regression on $\alpha$ and $\beta$ using the training dataset, which will give us the estimated value of two coefficients as well as the R-squared. The R-squared measures the strength of the relationship between the variable $\frac{d}{dt}LIT01(t)$ and two variables $LCV01D(t)$ and $FCV03D(t)$. The hypothetical invariant is only accepted if the R-squared value exceed a certain threshold. Otherwise, it implies that these devices do not show strong correlations that constitute a physical invariants.
% threshold determination

==> sections/experiment.tex <==
\begin{comment}
\section{Experiments}

In this section, we describe the specific experiments conducted using the methodology outlined above, including the details of the datasets and the specific invariants used.

\subsection{Invariant}

For our experiments, we used specific invariants detected in our study. Two examples of such invariants are:

\[
\text{LIT01} = \alpha \cdot \text{LCV01D} + \beta \cdot \text{FCV03D}
\]

\[
\text{LCV01D} = \alpha \cdot \text{PCV03D}
\]

where:
\begin{itemize}
    \item \textbf{LIT01}: Level Indicator Transmitter, indicating the water level in the return water tank.
    \item \textbf{LCV01D}: Level Control Valve, used to maintain the water level of the return water tank.
    \item \textbf{FCV03D}: Flow Control Valve, maintaining the outflow rate from the return water tank.
    \item \textbf{PCV03D}: Pressure Control Valve, controlling the pressure within the system.
    \item \(\alpha\) and \(\beta\): Coefficients determined through regression analysis.
    %\item \(f(\cdot)\): A function representing the relationship between variables.
\end{itemize}

In this experiment, we focus on the invariant:

\[
\text{LIT01} = \alpha \cdot \text{LCV01D} + \beta \cdot \text{FCV03D}
\]

For instance, in our experiments, we used the HAI dataset which contains four different versions (from 2019 to 2022), each with two different datasets. The first dataset represents normal behavior (Train file), while the second dataset contains data from periods where at least one attack occurred (Test file).

\subsection{Determine Window Size}

To determine the best sliding window size for our dataset versions, we used the method described in the methodology. By applying the 3-sigma rule and calculating the number of outlier data points, we identified the point where alpha and beta values stabilized. We then calculated the derivative of all points on the chart and selected the value closest to zero to ensure a balance between stability and anomaly detection. If the alpha and beta values differed, we calculated their average.

For example, in the 2020 version of the HAI dataset, which has three train files and five test files, we chose train1 and test5. We determined the window size using our defined method. In this case, the alpha window size is 3 and the beta window size is 6, with their average used as the final window size.

\begin{figure}[H]
    \centering
    \includegraphics[width=\linewidth]{images/windows_siza.png}
    \caption{Determination of optimal window size based on outlier counts and deviation sums for both alpha and beta coefficients.}
    \label{fig:window_size}
\end{figure}

\subsection{Detection Process}

For each version of the dataset, we conducted the following steps:\\
1. \textbf{Calculate Alpha and Beta for Train Files}: We extracted LIT01, FCV03D, and LCV01D from train1 to find the alpha and beta values for the train file using the linear regression model.\\
\begin{figure}[H]
    \centering
    \includegraphics[width=\linewidth]{images/train_alpha.png}
    \caption{Alpha values were calculated for the training dataset during the detection process.}
    \label{fig:train_alpha}
\end{figure}

2. \textbf{Determine Thresholds for Train Files}: After determining the alpha and beta for the train file, we set the thresholds. For alpha in the train dataset, the up threshold (\(\text{Up\_threshold\_alpha\_train}\)) is the highest alpha value, and the down threshold (\(\text{Down\_threshold\_alpha\_train}\)) is the lowest alpha value. Similarly, for beta in the train dataset, the up threshold (\(\text{Up\_threshold\_beta\_train}\)) is the highest beta value, and the down threshold (\(\text{Down\_threshold\_beta\_train}\)) is the lowest beta value.\\
3. \textbf{Calculate Alpha and Beta for Test Files}: We extracted LIT01, FCV03D, and LCV01D from test5 and found the alpha and beta values using the same linear regression model.\\
4. \textbf{Compare Alpha and Beta Values}: We compared the alpha and beta values of the test data with the thresholds from the training data. For every alpha\_test point, if the value exceeds the up threshold (\(\text{Up\_threshold\_alpha\_train}\)) or falls below the down threshold (\(\text{Down\_threshold\_alpha\_train}\)), we flagged it as an anomaly. Similarly, for every beta\_test point, if the value exceeds the up threshold (\(\text{Up\_threshold\_beta\_train}\)) or falls below the down threshold (\(\text{Down\_threshold\_beta\_train}\)), we flagged it as an anomaly.\\
\begin{figure}[H]
    \centering
    \includegraphics[width=\linewidth]{images/test_alpha.png}
    \caption{Comparison of alpha values for the test dataset against the determined thresholds.}
    \label{fig:test_file}
\end{figure}
5. \textbf{Combine Anomaly Points}: We combined all detected anomaly points from the comparisons to identify potential deviations from normal behavior.

\subsection{Evaluation}

We analyzed and interpreted the detected anomalies by sorting the anomaly points by time and grouping them based on time intervals. We then compared each group against a schedule of known attacks. If a group matched a known attack, it was considered a correctly predicted attack.

In our example, we detected the following attack times:

\begin{multicols}{2}
\begin{itemize}
    \item 2020-07-31 02:03:00
    \item 2020-07-31 04:30:15
    \item 2020-07-31 05:46:15
    \item 2020-07-31 09:55:00
    \item 2020-07-31 09:55:15
    \item 2020-07-31 09:55:30
    \item 2020-07-31 09:55:45
    \item 2020-07-31 09:56:00
    \item 2020-07-31 09:58:15
    \item 2020-07-31 09:58:15
    \item 2020-07-31 09:58:30
    \item 2020-07-31 09:58:45
    \item 2020-07-31 09:59:00
    \item 2020-07-31 09:59:15
    \item 2020-07-31 09:59:30
    \item 2020-07-31 09:59:45
    \item 2020-07-31 11:17:15
    \item 2020-07-31 11:17:30
    \item 2020-07-31 11:27:30
    \item 2020-07-31 11:27:45
\end{itemize}
\end{multicols}

These detected times were then classified into groups with a 60-second interval:

\begin{itemize}
    \item \textbf{G1}: 2020-07-31 02:03:00
    \item \textbf{G2}: 2020-07-31 04:30:15
    \item \textbf{G3}: 2020-07-31 05:46:15
    \item \textbf{G4}: 2020-07-31 09:55:00, 2020-07-31 09:55:15, 2020-07-31 09:55:30, 2020-07-31 09:55:45, 2020-07-31 09:56:00
    \item \textbf{G5}: 2020-07-31 09:58:15, 2020-07-31 09:58:15, 2020-07-31 09:58:30, 2020-07-31 09:58:45, 2020-07-31 09:59:00, 2020-07-31 09:59:15, 2020-07-31 09:59:30, 2020-07-31 09:59:45
    \item \textbf{G6}: 2020-07-31 11:17:15, 2020-07-31 11:17:30
    \item \textbf{G7}: 2020-07-31 11:27:30, 2020-07-31 11:27:45
\end{itemize}

We then cross-referenced these groups with theHAI dataset, which contains the exact attack times. Based on this comparison, we correctly detected attacks in G1, G4, and G5. These groups contained at least one attack that matched the known attack times in the HAI dataset.

By following this comprehensive methodology and conducting detailed experiments, we effectively detected and understood anomalies in CPS using LLMs and validated our findings through thorough data analysis and comparison with known attack scenarios.


By following this approach, the determined window size ensures a balance between capturing the dynamic behavior of the system and maintaining the ability to detect anomalies effectively.

Incorporation into the Anomaly Detection Process

The segmented data windows are then used in the anomaly detection process. Each window’s alpha and beta coefficients are compared against thresholds derived from training data to flag anomalies. This step-by-step process of segmenting the data, analyzing each window, and comparing it to expected norms is crucial for accurate and effective anomaly detection in Cyber-Physical Systems.

\end{comment}



    
\section{Experiments}

In this section, we describe the specific experiments conducted using the methodology outlined above, including the details of the datasets and the specific invariants used.

\subsection{Invariant}

For our experiments, we used specific invariants detected in our study. For better understanding, we used \(\alpha = k_1\) and \(\beta = k_2\). One example of such an invariant is:

\[
\text{LIT01} = \alpha \cdot \text{LCV01D} + \beta \cdot \text{FCV03D}
\]

where:
\begin{itemize}
    \item \textbf{LIT01}: Level Indicator Transmitter, indicating the water level in the return water tank.
    \item \textbf{LCV01D}: Level Control Valve, used to maintain the water level of the return water tank.
    \item \textbf{FCV03D}: Flow Control Valve, maintaining the outflow rate from the return water tank.
    \item \(\mathbf{C}\): Vectors of coefficients \([\alpha, \beta]\).
\end{itemize}

For our experiments, we used the HAI dataset, which contains four different versions (from 2019 to 2022), each with two different datasets. The first dataset represents normal behavior (Train file), while the second dataset contains data from periods where at least one attack occurred (Test file).

\subsection{Determine Window Size}

To determine the best sliding window size for our dataset versions, we used the method described in the methodology. By applying the 3-sigma rule and calculating the number of outlier data points, we identified the point where alpha and beta values stabilized. We then calculated the derivative of all points on the chart and selected the value closest to zero to ensure a balance between stability and anomaly detection. If the alpha and beta values differed, we calculated their average.

For example, in the 2020 version of the HAI dataset, which has three train files and five test files, we chose train1 and test5. We determined the window size using our defined method. In this case, the alpha window size is 3 and the beta window size is 6, with their average used as the final window size:

\[
\text{Window Size} = \frac{3 + 6}{2} = 4.5 \approx 5 \text{ (minutes)}
\]

\begin{figure}[H]
    \centering
    \includegraphics[width=\linewidth]{images/windows_siza.png}
    \caption{Determination of optimal window size based on outlier counts and deviation sums for both alpha and beta coefficients.}
    \label{fig:window_size}
\end{figure}

\subsection{Detection Process}

For each version of the dataset, we conducted the following steps:

\begin{enumerate}
    \item \textbf{Calculate Alpha and Beta for Train Files}: Extract LIT01, FCV03D, and LCV01D from train1 to find the alpha and beta values for the train file using the linear regression model.
    \[
    \hat{\alpha}_{train}, \hat{\beta}_{train}
    \]
    
    \begin{figure}[H]
        \centering
        \includegraphics[width=\linewidth]{images/train1.png}
        \caption{Alpha values calculated for the training dataset during the detection process.}
        \label{fig:train_alpha}
    \end{figure}
    
    \item \textbf{Determine Thresholds for Train Files}: After determining the alpha and beta for the train file, set the thresholds. For alpha in the train dataset, the up threshold \footnote{\(\text{Up\_threshold\_alpha\_train}\)} is the highest alpha value, and the down threshold \footnote{\(\text{Down\_threshold\_alpha\_train}\)} is the lowest alpha value. Similarly, for beta in the train dataset, the up threshold \footnote{\(\text{Up\_threshold\_beta\_train}\)} is the highest beta value, and the down threshold \footnote{\(\text{Down\_threshold\_beta\_train}\)} is the lowest beta value.
    \[
    \text{Threshold}_{\alpha} = [\alpha_{min}, \alpha_{max}] \quad \text{and} \quad \text{Threshold}_{\beta} = [\beta_{min}, \beta_{max}]
    \]

    \item \textbf{Calculate Alpha and Beta for Test Files}: Extract LIT01, FCV03D, and LCV01D from test5 and find the alpha and beta values using the same linear regression model.
    \[
    \hat{\alpha}_{test}, \hat{\beta}_{test}
    \]
    
    \item \textbf{Compare Alpha and Beta Values}: Compare the alpha and beta values of the test data with the thresholds from the training data. For every alpha\_test point, if the value exceeds the up threshold (\(\text{Up\_threshold\_alpha\_train}\)) or falls below the down threshold (\(\text{Down\_threshold\_alpha\_train}\)), flag it as an anomaly. Similarly, for every beta\_test point, if the value exceeds the up threshold (\(\text{Up\_threshold\_beta\_train}\)) or falls below the down threshold (\(\text{Down\_threshold\_beta\_train}\)), flag it as an anomaly.
    \[
    \text{Anomaly if} \quad \hat{\alpha}_{test} \notin \text{Threshold}_{\alpha} \quad \text{or} \quad \hat{\beta}_{test} \notin \text{Threshold}_{\beta}
    \]
    
    \begin{figure}[H]
        \centering
        \includegraphics[width=\linewidth]{images/test1.png}
        \caption{Comparison of alpha values for the test dataset against the determined thresholds.}
        \label{fig:test_file}
    \end{figure}
    
    \item \textbf{Combine Anomaly Points}: Combine all detected anomaly points from the comparisons to identify potential deviations from normal behavior.
    \[
    \text{Anomaly Points} = \{t | \hat{\alpha}_t \notin \text{Threshold}_{\alpha} \text{ or } \hat{\beta}_t \notin \text{Threshold}_{\beta}\}
    \]
\end{enumerate}

\subsection{Evaluation}

We analyzed and interpreted the detected anomalies by sorting the anomaly points by time and grouping them based on time intervals. We then compared each group against a schedule of known attacks. If a group matched a known attack, it was considered a correctly predicted attack.

In our example, we detected the following attack times:

\begin{table}[h]
\centering
\caption{Detected Attack Times}
\begin{tabular}{l}
\hline
\textbf{Detected Attack Times} \\ \midrule
2020-07-31 02:03:00          \\ \midrule
2020-07-31 04:30:15          \\ \midrule
2020-07-31 05:46:15          \\ \midrule
2020-07-31 09:55:00          \\ \midrule
2020-07-31 09:55:15          \\ \midrule
2020-07-31 09:55:30          \\ \midrule
2020-07-31 09:55:45          \\ \midrule
2020-07-31 09:56:00          \\ \midrule
2020-07-31 09:58:15          \\ \midrule
2020-07-31 09:58:30          \\ \midrule
2020-07-31 09:58:45          \\ \midrule
2020-07-31 09:59:00          \\ \midrule
2020-07-31 09:59:15          \\ \midrule
2020-07-31 09:59:30          \\ \midrule
2020-07-31 09:59:45          \\ \midrule
2020-07-31 11:17:15          \\ \midrule
2020-07-31 11:17:30          \\ \midrule
2020-07-31 11:27:30          \\ \midrule
2020-07-31 11:27:45          \\ \midrule
\end{tabular}
\end{table}

These detected times were then classified into groups with a 60-second interval:

\begin{table}[h]
\centering
\caption{Grouped Detected Times}
\begin{tabular}{c|p{6.5cm}}
\hline
\textbf{Group} & \textbf{Detected Times} \\ \midrule
G1             & 2020-07-31 02:03:00     \\ \midrule
G2             & 2020-07-31 04:30:15     \\ \midrule
G3             & 2020-07-31 05:46:15     \\ \midrule
G4             & 2020-07-31 09:55:00, 2020-07-31 09:55:15, 2020-07-31 09:55:30, 2020-07-31 09:55:45, 2020-07-31 09:56:00 \\ \midrule
G5             & 2020-07-31 09:58:15, 2020-07-31 09:58:30, 2020-07-31 09:58:45, 2020-07-31 09:59:00, 2020-07-31 09:59:15, 2020-07-31 09:59:30, 2020-07-31 09:59:45 \\ \midrule
G6             & 2020-07-31 11:17:15, 2020-07-31 11:17:30 \\ \midrule
G7             & 2020-07-31 11:27:30, 2020-07-31 11:27:45 \\ \midrule
\end{tabular}
\end{table}

We then cross-referenced these groups with the HAI dataset, which contains the exact attack times. Based on this comparison, we correctly detected attacks in G1, G4, and G5. These groups contained at least one attack that matched the known attack times in the HAI dataset.
\begin{table}[h]
\centering
\caption{Evaluation Results}
\begin{tabular}{c|c}
\hline
\textbf{Group} & \textbf{Correctly Detected} \\ \midrule
G1             & Yes                         \\ \midrule
G2             & No                          \\ \midrule
G3             & No                          \\ \midrule
G4             & Yes                         \\ \midrule
G5             & Yes                         \\ \midrule
G6             & No                          \\ \midrule
G7             & No                          \\ \midrule
\end{tabular}
\end{table}
By following this comprehensive methodology and conducting detailed experiments, we effectively detected and understood anomalies in CPS using LLMs and validated our findings through thorough data analysis and comparison with known attack scenarios.


==> sections/methodology.tex <==
\section{Methodology}

In this section, we describe the step-by-step methodology used for anomaly detection in Cyber-Physical Systems (CPS) using Large Language Models (LLMs). The purpose of this study is to enhance the detection of anomalies in CPS by leveraging LLMs to automate the extraction of physical invariants, validate these invariants, and use them for anomaly detection.

\subsection{Hypothetical Invariants Extraction}

The first step in our methodology aims to identifying some hypothetical invariants by leveraging the power of large language models. 



identifying physical invariants using LLMs. Physical invariants are relationships that hold true under normal operating conditions of the CPS. These invariants can take various forms and involve different numbers of variables. They are expressed as equations involving multiple variables, coefficients, and functions.

For example, some of the invariants we identified are:

\[
\text{LIT01} = \alpha \cdot \text{LCV01D} + \beta \cdot \text{FCV03D}
\]

\[
\text{LCV01D} = \alpha \cdot \text{PCV03D}
\]

where:
\begin{itemize}
    \item \textbf{LIT01}: Level Indicator Transmitter, indicating the water level in the return water tank.
    \item \textbf{LCV01D}: Level Control Valve, used to maintain the water level of the return water tank.
    \item \textbf{FCV03D}: Flow Control Valve, maintaining the outflow rate from the return water tank.
    \item \textbf{PCV03D}: Pressure Control Valve, controlling the pressure within the system.
    \item \(\alpha\) and \(\beta\): Coefficients determined through regression analysis.
    ‌%\item \(f(\cdot)\): A function representing the relationship between variables.
\end{itemize}

\textbf{Calculation of Alpha and Beta}

The steps to calculate alpha and beta involve:

1. \textbf{Data Preparation}: Identify the independent variables (\(X\)) and the dependent variable (\(y\)). The derivative of the dependent variable is often used to capture the rate of change influenced by the independent variables.

2. \textbf{Adding a Constant Term}: To account for the intercept (\(\alpha\)) in the linear regression model, a constant term is added to the independent variables by augmenting the dataset with an additional column of ones.

3. \textbf{Fitting the Linear Regression Model}: Using the prepared data, fit an Ordinary Least Squares (OLS) regression model. OLS regression finds the best-fitting line through the data points by minimizing the sum of squared residuals.

4. \textbf{Extracting Coefficients}: After fitting the model, extract the coefficients for the independent variables. The intercept term represents alpha (\(\alpha\)), and the slope coefficients represent beta (\(\beta\)).

For given window of data, the regression model equation is:

\[
y = \alpha + \beta_1 \cdot X_1 + \beta_2 \cdot X_2 + \epsilon
\]

where \(\alpha\) is the intercept, \(\beta_1\) and \(\beta_2\) are the coefficients for the independent variables, and \(\epsilon\) is the error term representing the difference between observed and predicted values.

\subsection{Sliding Window Method}

To accurately detect anomalies in CPS using LLMs, it is crucial to segment the data into manageable time frames. This segmentation is achieved by defining a rolling window, specified in minutes, over which certain calculations or models are applied. The variable window\_size\_minutes plays a vital role in this process.

\textbf{Definition and Purpose}

The window\_size\_minutes variable defines the duration of each window in minutes. For example, if window\_size\_minutes is set to 30, it indicates that each window spans 30 minutes. The primary purpose of using window\_size\_minutes is to segment the time-series data into chunks of specified length, allowing for detailed analysis within each segment. This approach is beneficial for detecting patterns, trends, and anomalies that may not be apparent in the entire dataset.

\textbf{Implementation in the Analysis Process}

The window\_size\_minutes variable is used in conjunction with other parameters like the stride (the interval at which windows start) to generate a sequence of timestamps that represent the starting points of each window. Here’s a detailed breakdown of its implementation:

1. \textbf{Conversion to Seconds and End Time Calculation}: The duration specified by window\_size\_minutes is converted to seconds to define the end time for processing the data. This ensures that the time calculations are precise and consistent.

2. \textbf{Generating Timestamps}: The variable is used along with the stride to create a range of timestamps, representing the starting points of each window. This helps in segmenting the data into continuous, overlapping, or non-overlapping windows, depending on the stride value.

3. \textbf{Segmentation for Model Fitting and Analysis}: Each window of data, determined by window\_size\_minutes, is used to fit models such as Ordinary Least Squares (OLS) regression, calculate derivatives, or perform other statistical analyses. By examining these smaller segments, the analysis can detect subtle changes and patterns that might be missed in a broader overview.

\textbf{Balancing Stability and Anomaly Detection}

Choosing an appropriate window size is critical to balance the stability of calculated coefficients (alpha and beta) with the ability to detect anomalies. Larger window sizes result in more stable coefficients due to increased data points but may dilute anomalies, making them harder to detect. Conversely, smaller window sizes increase sensitivity to anomalies but can result in more volatile coefficient estimates.

To determine the optimal window size, the methodology involves:

1. \textbf{Applying the 3-Sigma Rule}: By applying the 3-sigma rule, data points falling outside the +/- 3-sigma range are identified as potential anomalies. This helps in understanding how alpha and beta values stabilize as the window size changes.

2. \textbf{Calculating Derivatives}: The derivatives of data points on the chart are calculated to identify where the values stabilize. The window size closest to zero derivative is selected to balance stability and anomaly detection.

By following this approach, the determined window size ensures a balance between capturing the dynamic behavior of the system and maintaining the ability to detect anomalies effectively.

\subsection{Detection Process}

The process for detecting anomalies involves several steps:

1. \textbf{Calculate Alpha and Beta for Training Data}: Calculate the alpha and beta values for the training data by fitting a linear regression model.

2. \textbf{Determine Thresholds for Training Data}: Determine the thresholds for alpha and beta values in the training data. These thresholds represent the expected range of values under normal operating conditions.

3. \textbf{Calculate Alpha and Beta for Test Data}: Calculate the alpha and beta values for the test data using the same linear regression model.

4. \textbf{Compare Alpha and Beta Values}: Compare the alpha and beta values of the test data with the thresholds from the training data. Flag any values that fall outside the thresholds as anomalies.

5. \textbf{Combine Anomaly Points}: Combine all detected anomaly points from the comparisons to identify potential deviations from normal behavior.

\subsection{Evaluation}

In the evaluation phase, we analyze and interpret the detected anomalies to ensure they are accurately identified and classified. 

First, we sort the detected anomaly points by time to ensure they are in chronological order. Sorting the data points allows us to identify patterns and temporal relationships among the anomalies. 

Next, we classify the sorted anomaly points by grouping them based on time intervals. The first data point starts a new group, and subsequent points are added to the group if they occur within a specified time interval, typically 60 seconds, of the previous point. If a point occurs outside this interval, a new group is created. This grouping helps in consolidating multiple anomaly points that are closely related in time, indicating a single anomalous event.

Once the groups are formed, we evaluate the detected anomalies by comparing each group against a schedule of known attacks. The schedule of known attacks contains the timestamps and descriptions of attacks that occurred during the test period. By matching the detected groups with the known attacks, we can determine the accuracy of our anomaly detection method. If a group matches a known attack, it is considered a correctly predicted attack. This step is crucial for validating our detection method and understanding its effectiveness in identifying real anomalies.




\section{Methodology}

In this section, we describe the methodology used for anomaly detection in Cyber-Physical Systems (CPS) using Large Language Models (LLMs). Our goal is to enhance anomaly detection by leveraging LLMs to automate the extraction of physical invariants, validate these invariants, and use them for detecting anomalies.

\subsection{Invariants Extraction}

The first step in our methodology involves identifying physical invariants using LLMs. Physical invariants are consistent relationships that hold true under normal operating conditions of the CPS. These invariants can be expressed as equations involving multiple variables, coefficients, and functions, and are essential for understanding the system's normal behavior.

For example, some of the invariants identified are:

\[
\text{LIT01} = \alpha \cdot \text{LCV01D} + \beta \cdot \text{FCV03D}
\]

\[
\text{LCV01D} = \alpha \cdot \text{PCV03D}
\]

where:
\begin{itemize}
    \item \textbf{LIT01}: Level Indicator Transmitter, indicating the water level in the return water tank.
    \item \textbf{LCV01D}: Level Control Valve, used to maintain the water level of the return water tank.
    \item \textbf{FCV03D}: Flow Control Valve, maintaining the outflow rate from the return water tank.
    \item \textbf{PCV03D}: Pressure Control Valve, controlling the pressure within the system.
    \item \(\alpha\) and \(\beta\): Coefficients determined through regression analysis.
\end{itemize}

\textbf{Calculation of Alpha and Beta}

The steps to calculate \(\alpha\) and \(\beta\) are as follows:

\begin{enumerate}
    \item \textbf{Data Preparation}: Identify the independent variables (\(X\)) and the dependent variable (\(y\)). Often, the rate of change of the dependent variable is used to capture the influence of the independent variables. The relationship can be described by the following equation:
    \[
    y_t = f(X_t) + \epsilon_t
    \]
    where \(y_t\) is the dependent variable at time \(t\), \(X_t\) are the independent variables, and \(\epsilon_t\) is the error term.
    
    \item \textbf{Adding a Constant Term}: To account for the intercept (\(\alpha\)) in the linear regression model, add a column of ones to the dataset as a constant term. This can be represented as:
    \[
    X' = [1, X]
    \]
    where \(X'\) is the augmented matrix with the constant term.

    \item \textbf{Fitting the Linear Regression Model}: Fit an Ordinary Least Squares (OLS) regression model to the prepared data. This model finds the best-fitting line by minimizing the sum of squared residuals between observed and predicted values. The OLS solution can be found using:
    \[
    \hat{\beta} = (X'X)^{-1}X'y
    \]
    where \(\hat{\beta}\) are the estimated coefficients.

    \item \textbf{Extracting Coefficients}: After fitting the model, extract the coefficients for the independent variables. The intercept term represents \(\alpha\), and the slope coefficients represent \(\beta\).
\end{enumerate}

For a given window of data, the regression model equation is:

\[
y = \alpha + \beta_1 \cdot X_1 + \beta_2 \cdot X_2 + \epsilon
\]

where \(\alpha\) is the intercept, \(\beta_1\) and \(\beta_2\) are the coefficients for the independent variables, and \(\epsilon\) is the error term representing the difference between observed and predicted values.

\subsection{Sliding Window Method}

To accurately detect anomalies in CPS, it is crucial to segment the data into manageable time frames using a rolling window, specified in minutes. The variable \textit{window\_size\_minutes} plays a vital role in this process.

\textbf{Definition and Purpose}

The \textit{window\_size\_minutes} variable defines the duration of each window in minutes. For example, if \textit{window\_size\_minutes} is set to 30, it means each window spans 30 minutes. This segmentation allows for detailed analysis within each segment, aiding in detecting patterns, trends, and anomalies that may not be apparent in the entire dataset.

\textbf{Implementation in the Analysis Process}

The \textit{window\_size\_minutes} variable is used along with the stride (the interval at which windows start) to generate a sequence of timestamps representing the starting points of each window:

\begin{enumerate}
    \item \textbf{Conversion to Seconds and End Time Calculation}: Convert the \textit{window\_size\_minutes} duration to seconds to define the end time for processing the data accurately.
    \[
    \text{end\_time} = \text{start\_time} + \text{window\_size\_minutes} \times 60
    \]

    \item \textbf{Generating Timestamps}: Use the \textit{window\_size\_minutes} and stride to create a range of timestamps, segmenting the data into continuous, overlapping, or non-overlapping windows. 
    \[
    \text{timestamps} = [t_0, t_1, t_2, \ldots, t_n]
    \]
    where \(t_{i+1} = t_i + \text{stride}\).

    \item \textbf{Segmentation for Model Fitting and Analysis}: Each window of data, defined by \textit{window\_size\_minutes}, is used to fit models like OLS regression or perform other statistical analyses.
\end{enumerate}

\textbf{Balancing Stability and Anomaly Detection}

Choosing an appropriate window size balances the stability of calculated coefficients (\(\alpha\) and \(\beta\)) with the ability to detect anomalies. Larger window sizes result in more stable coefficients due to more data points but may dilute anomalies, making them harder to detect. Conversely, smaller window sizes increase sensitivity to anomalies but can result in more volatile coefficient estimates.

To determine the optimal window size, the methodology involves:

\begin{enumerate}
    \item \textbf{Applying the 3-Sigma Rule}: Identify data points falling outside the +/- 3-sigma range as potential anomalies. This helps in understanding how \(\alpha\) and \(\beta\) values stabilize as the window size changes.
    \[
    \mu \pm 3\sigma
    \]
    where \(\mu\) is the mean and \(\sigma\) is the standard deviation of the coefficients.

    \item \textbf{Calculating Derivatives}: Calculate the derivatives of data points to identify where the values stabilize. Select the window size where the derivative is closest to zero to balance stability and anomaly detection.
    \[
    \frac{d\alpha}{dt} \approx 0 \quad \text{and} \quad \frac{d\beta}{dt} \approx 0
    \]
\end{enumerate}

\subsection{Detection Process}

The anomaly detection process involves several steps:

\begin{enumerate}
    \item \textbf{Calculate Alpha and Beta for Training Data}: Fit a linear regression model to calculate the \(\alpha\) and \(\beta\) values for the training data.
    \[
    \hat{\alpha}_{train}, \hat{\beta}_{train}
    \]

    \item \textbf{Determine Thresholds for Training Data}: Establish thresholds for \(\alpha\) and \(\beta\) values in the training data, representing the expected range under normal operating conditions.
    \[
    \text{Threshold}_{\alpha} = [\alpha_{min}, \alpha_{max}] \quad \text{and} \quad \text{Threshold}_{\beta} = [\beta_{min}, \beta_{max}]
    \]

    \item \textbf{Calculate Alpha and Beta for Test Data}: Calculate the \(\alpha\) and \(\beta\) values for the test data using the same linear regression model.
    \[
    \hat{\alpha}_{test}, \hat{\beta}_{test}
    \]

    \item \textbf{Compare Alpha and Beta Values}: Compare the \(\alpha\) and \(\beta\) values of the test data with the thresholds from the training data. Flag values falling outside the thresholds as anomalies.
    \[
    \text{Anomaly if} \quad \hat{\alpha}_{test} \notin \text{Threshold}_{\alpha} \quad \text{or} \quad \hat{\beta}_{test} \notin \text{Threshold}_{\beta}
    \]

    \item \textbf{Combine Anomaly Points}: Combine detected anomaly points to identify potential deviations from normal behavior.
    \[
    \text{Anomaly Points} = \{t | \hat{\alpha}_t \notin \text{Threshold}_{\alpha} \text{ or } \hat{\beta}_t \notin \text{Threshold}_{\beta}\}
    \]
\end{enumerate}

\subsection{Evaluation}

In the evaluation phase, detected anomalies are analyzed and interpreted to ensure accurate identification and classification:

\begin{enumerate}
    \item \textbf{Sort Anomaly Points by Time}: Sort detected anomaly points chronologically to identify patterns and temporal relationships.
    \[
    \text{Sorted Anomalies} = \text{sort}(\text{Anomaly Points})
    \]

    \item \textbf{Classify Anomaly Points}: Group anomaly points based on time intervals. Points occurring within a specified interval (e.g., 60 seconds) of the previous point are grouped together, indicating a single anomalous event.
    \[
    \text{Group}_{i} = \{t_j \mid t_j - t_{j-1} \leq 60 \text{ seconds}\}
    \]

    \item \textbf{Compare with Known Attacks}: Evaluate detected anomalies by comparing each group against a schedule of known attacks. Match detected groups with known attacks to determine the accuracy of the anomaly detection method.
    \[
    \text{Accuracy} = \frac{\text{True Positives}}{\text{True Positives} + \text{False Positives} + \text{False Negatives}}
    \]
\end{enumerate}

By following this methodology, we ensure a systematic approach to detect anomalies in CPS, leveraging the power of LLMs for automated extraction and validation of physical invariants.








\section{Methodology}

In this section, we describe the methodology used for anomaly detection in Cyber-Physical Systems (CPS) using Large Language Models (LLMs). Our goal is to enhance anomaly detection by leveraging LLMs to automate the extraction of physical invariants, validate these invariants, and use them for detecting anomalies.

\subsection{Invariants Extraction}

The first step in our methodology involves identifying physical invariants using LLMs. Physical invariants are consistent relationships that hold under normal operating conditions of the CPS. These invariants can be expressed as equations involving multiple variables, coefficients, and functions, and are essential for understanding the system's normal behavior.



\textbf{Definition of Invariants:} Physical invariants are mathematical expressions that represent the constant relationships between various state variables of a system under normal operating conditions. These invariants help understand the system's standard operational behavior.

\textbf{Overall Shape of the Invariants:} The general form of the invariants can be represented as:
\[
\mathbf{A} \cdot \mathbf{X} = \mathbf{B}
\]
where \( \mathbf{A} \) is a matrix of coefficients, \( \mathbf{X} \) is a vector of state variables, and \( \mathbf{B} \) is a vector of constants.


The following invariants are identified in our study as the outputs of the LLM:

$$
\frac{d(\text{LIT01})}{dt} = k_1 \cdot \text{FCV03D} - k_2 \cdot \text{LCV01D}
$$
$$
\text{LCV01D} = k_3 \cdot \text{PCV03D}
$$
$$
\text{PIT01} = k_4 \cdot \text{PCV01D} + k_5 \cdot \text{PCV02D}
$$
$$
\text{FT03Z} = k_6 \cdot \text{FT03}
$$
$$
\text{LCV01D} = k_7 \cdot \text{FCV03D}
$$
\[
\frac{d(\text{LIT01})}{dt} = \frac{k_8}{A_t} \cdot \text{LCV01D} - \frac{k_{9}}{A_t} \cdot \text{FCV03D}
\]
$$
\text{FT03} = k_{8} \cdot \text{FCV03D}
$$
$$
\text{TIT01} = k_{9} \cdot \text{FCV01D} + k_{10} \cdot \text{FCV02D}
$$


\begin{table}[h!]
\centering
\begin{tabular}{c|p{6.5cm}}
\hline
\textbf{Variable} & \textbf{Description} \\ \midrule
LIT01 & Level Indicator Transmitter, indicating the water level of the return water tank (TK03). \\ \midrule
LCV01D & Level Control Valve, used to maintain the water level of the return water tank (TK03). \\ \midrule
FCV03D & Flow Control Valve, controlling the outflow rate from the return water tank (TK03). \\ \midrule
FCV01D & Flow Control Valve, controlling the flow rate into the main water tank. \\ \midrule
FCV02D & Flow Control Valve, controlling the flow rate out of the main water tank. \\ \midrule
PCV03D & Pressure Control Valve, controlling the pressure within the system. \\ \hline
PCV01D & Pressure Control Valve, maintaining the pressure between the main and return water tanks. \\ 
PCV02D & Another Pressure Control Valve, maintaining the pressure between the main and return water tanks. \\ \midrule
PIT01 & Pressure Indicator Transmitter, indicating the pressure at the heat-exchanger outlet. \\ \midrule
FT03 & Flow Transmitter, measuring the flow rate of the return water tank (TK03). \\ \midrule
FT03Z & Converted flow rate measurement from FT03, in liters per hour. \\ \midrule
TIT01 & Temperature Indicator Transmitter, indicating the temperature in the system. \\ \midrule
A\_t & Cross-sectional area of the tank.\\ \midrule
\end{tabular}
\caption{Description of Variables}
\label{tab:variables}
\end{table}
\end{comment}




    

\subsubsection{Calculation of Coefficient Vectors}

The steps to calculate the coefficient vectors are as follows:

\begin{enumerate}
    \item \textbf{Data Preparation}: Identify the independent variables (\(\mathbf{X}\)) and the dependent variable (\(\mathbf{y}\)). Often, the rate of change of the dependent variable is used to capture the influence of the independent variables. The relationship can be described by the following equation:
    \[
    \mathbf{y}_t = f(\mathbf{X}_t) + \epsilon_t
    \]
    where \(\mathbf{y}_t\) is the dependent variable at time \(t\), \(\mathbf{X}_t\) are the independent variables, and \(\epsilon_t\) is the error term.
    
    \item \textbf{Adding a Constant Term}: To account for the intercept in the linear regression model, add a column of ones to the dataset as a constant term. This can be represented as:
    \[
    \mathbf{X}' = [1, \mathbf{X}]
    \]
    where \(\mathbf{X}'\) is the augmented matrix with the constant term.

    \item \textbf{Fitting the Linear Regression Model}: Fit an Ordinary Least Squares (OLS) regression model to the prepared data. This model finds the best-fitting line by minimizing the sum of squared residuals between observed and predicted values. The OLS solution can be found using:
    \[
    \hat{\mathbf{C}} = (\mathbf{X}'\mathbf{X})^{-1}\mathbf{X}'\mathbf{y}
    \]
    where \(\hat{\mathbf{C}}\) are the estimated coefficients.

    \item \textbf{Extracting Coefficients}: After fitting the model, extract the coefficients for the independent variables. The intercept term represents the constant, and the slope coefficients represent the other terms in the vector.
\end{enumerate}

For a given window of data, the regression model equation is:

\[
\mathbf{y} = \alpha + \mathbf{C} \cdot \mathbf{X} + \epsilon
\]

where \(\alpha\) is the intercept, \(\mathbf{C}\) is the vector of coefficients for the independent variables, and \(\epsilon\) is the error term representing the difference between observed and predicted values.



   
\subsection{Detection Process}

The anomaly detection process involves several steps:

\begin{enumerate}
    \item \textbf{Calculate Coefficients for Training Data}: Fit a linear regression model to calculate the coefficient values for the training data.
    \[
    \hat{\mathbf{C}}_{\text{train}}
    \]

    \item \textbf{Determine Thresholds for Training Data}: Establish thresholds for the coefficient values in the training data, representing the expected range under normal operating conditions.
    \[
    \text{Threshold}_{\mathbf{C}} = [\mathbf{C}_{\text{min}}, \mathbf{C}_{\text{max}}]
    \]

    \item \textbf{Calculate Coefficients for Test Data}: Calculate the coefficient values for the test data using the same linear regression model.
    \[
    \hat{\mathbf{C}}_{\text{test}}
    \]

    \item \textbf{Compare Coefficient Values}: Compare the coefficient values of the test data with the thresholds from the training data. Flag values falling outside the thresholds as anomalies.
    \[
    \text{Anomaly if} \quad \hat{\mathbf{C}}_{\text{test}} \notin \text{Threshold}_{\mathbf{C}}
    \]

    \item \textbf{Combine Anomaly Points}: Combine detected anomaly points to identify potential deviations from normal behavior.
    \[
    \text{Anomaly Points} = \{t \mid \hat{\mathbf{C}}_t \notin \text{Threshold}_{\mathbf{C}}\}
    \]
\end{enumerate}


\subsection{Evaluation}

In the evaluation phase, detected anomalies are analyzed and interpreted to ensure accurate identification and classification:

\begin{enumerate}
    \item \textbf{Sort Anomaly Points by Time}: Sort detected anomaly points chronologically to identify patterns and temporal relationships.
    \[
    \text{Sorted Anomalies} = \text{sort}(\text{Anomaly Points})
    \]

    \item \textbf{Classify Anomaly Points}: Group anomaly points based on time intervals. Points occurring within a specified interval (e.g., 60 seconds) of the previous point are grouped together, indicating a single anomalous event.
    \[
    \text{Group}_{i} = \{t_j \mid t_j - t_{j-1} \leq 60 \text{ seconds}\}
    \]

    \item \textbf{Compare with Known Attacks}: Evaluate detected anomalies by comparing each group against a schedule of known attacks. Match detected groups with known attacks to determine the accuracy of the anomaly detection method.
    \[
    \text{Accuracy} = \frac{\text{True Positives}}{\text{True Positives} + \text{False Positives} + \text{False Negatives}}
    \]
\end{enumerate}

By following this methodology, we ensure a systematic approach to detect anomalies in CPS, leveraging the power of LLMs for automated extraction and validation of physical invariants.


==> sections/related_old.tex <==
\section{Related Works}\label{sec:related}

\subsection{Anomaly Detection using Physical Invariants}

Anomaly detection in CPS often utilizes physical invariants—relationships or conditions derived from the system's governing physical laws that indicate proper functioning. These invariants serve as a baseline for identifying anomalies signaling faults or cyber-attacks. One approach applied unsupervised machine learning to detect anomalies in electrical substations by inferring physical invariants from data rather than explicitly encoding laws like Kirchhoff's, demonstrating flexibility in recognizing system states \cite{b1}. Similarly, a log-based anomaly detection method using the Local Outlier Factor (LOF) algorithm identified control system failures in an aquarium management system, leveraging physical invariants in log data \cite{b2}.
In smart grids, the IREST sensor combined cyber and physical features to detect anomalies, validated using the ISAAC testbed to differentiate between cyber and physical disturbances \cite{b3}. A Spatiotemporal Graphical Model captured dependencies in CPS data, incorporating physical invariants to detect subtle anomalies across distributed systems \cite{b4}. Another study used unsupervised learning to model normal operational patterns and detect anomalies in smart grids, emphasizing the role of physical invariants in security \cite{b5}. 
A survey on smart grid security underscored the importance of physical invariants for stability, discussing machine learning and blockchain as tools to enhance anomaly detection \cite{b6}. In smart water infrastructure, a machine learning framework combined physical rules with anomaly detection techniques, demonstrating effective identification of cyber and physical threats \cite{b7}. A spatiotemporal model for distributed CPS improved anomaly detection by understanding the physical laws governing the systems \cite{b8}.
In advanced driver assistance systems, integrating deep learning with physical invariants enhanced detection accuracy and reduced false positives \cite{b9}. A hybrid approach combined statistical methods and machine learning, explicitly incorporating physical invariants to detect anomalies in complex industrial processes \cite{b11}. 
Few-shot learning with a Siamese Neural Network leveraged physical invariants for better generalization in industrial CPS with limited data \cite{b12}. RNNs for anomaly detection in CPS improved accuracy across various conditions by integrating invariants \cite{b13}. Privacy-preserving frameworks further used physical invariants to enhance detection while safeguarding sensitive information \cite{b14, b26, b19, b27}.

\subsection{Causal Discovery for Anomaly Detection}

Causal discovery has gained increasing attention in anomaly detection by uncovering the underlying cause-effect relationships in temporal data. Traditional anomaly detection methods primarily rely on statistical deviations, whereas causal discovery offers a more structured approach to identifying the root causes of anomalies, improving interpretability and robustness. Graph-based causal discovery has been instrumental in advancing anomaly detection. Attention-based models dynamically infer causal dependencies among multivariate time series, leveraging graph learning and multi-head attention mechanisms. Recent work introduced a multimodal spatial–temporal graph attention network (MST-GAT) to enhance causal discovery for anomaly detection in CPS \cite{MST-GAT}. Similarly, methods such as Graph Neural Network-based Anomaly Detection (GDN) utilize attention weights to represent sensor dependencies, improving anomaly attribution \cite{GDN}.

Beyond attention mechanisms, Granger causality-based methods provide a foundation for causal inference in time-series anomaly detection. These approaches analyze temporal dependencies to uncover causal structures, which are particularly useful for modeling complex interactions in sensor networks \cite{GrangerDeep}. Recent advances integrate deep learning with Granger causality to improve scalability in high-dimensional settings \cite{FuSAGNet}. Structural learning-based causal discovery also plays a significant role in anomaly detection. Techniques leveraging Structural Causal Models (SCMs) construct causal graphs that differentiate between spurious correlations and true causal dependencies, which is crucial for diagnosing system faults in cyber-physical environments \cite{causal_disc}.

Recent studies emphasize the integration of causal discovery with deep anomaly detection to enhance decision-making and reduce false positives. By uncovering the root causes of anomalies, these methods contribute to more interpretable and effective anomaly detection frameworks. Given the growing complexity of CPS, causal discovery continues to be an essential research direction for advancing anomaly detection.

\subsection{LLM-based Anomaly Detection}
% https://arxiv.org/pdf/2402.10350v1.pdf

Recent advancements in anomaly detection for CPS and video surveillance leverage Large Language Models (LLMs). For Video Anomaly Detection (VAD), VLLMs like VAD-LLaMA detect anomalies in surveillance footage and provide textual explanations, improving upon traditional methods \cite{b33}.
In CPS, LLMs automate the extraction of physical invariants, streamlining anomaly detection and reducing manual effort \cite{b31}. This technique has been extended to Industrial Control Systems (ICS) for scalable monitoring with minimal domain expertise \cite{b32,alam2024assess}. In smart grids, combining LLMs with statistical analysis improves real-time anomaly detection by integrating historical data with sensor inputs \cite{b30,rashvand2024enhancing}. Additionally, LLMs simplify invariant extraction, enhancing usability for large-scale deployments \cite{b20}.
LLMs such as GPT-4 enhance CPS resilience and adaptability. A proposed framework addresses challenges like context grounding and formal verification for reliable LLM deployment in deterministic environments \cite{b15}. The concept of "Penetrative AI" shows LLMs interpreting IoT sensor data for real-time monitoring in complex environments \cite{b16}.
Integrating LLMs with Programmable Logic Controllers (PLCs) in industrial CPS enables real-time anomaly diagnosis, critical for rapid response environments \cite{b18}. Furthermore, robust assurance frameworks are needed to mitigate risks associated with LLM deployment in CPS \cite{b19}. 
A systematic review highlights challenges in LLM applications for forecasting and anomaly detection, such as dataset reliance, generalizability issues, and computational demands, offering insights for optimizing LLM use in CPS \cite{b20,zibaeirad2024vulnllmeval}.

Our approach leverages Large Language Models (LLMs) to automatically extract and validate physical invariants from CPS documentation, reducing the need for domain expertise and improving scalability. Unlike existing methods, \textit{AnomalyLLM} integrates LLM-driven invariant extraction directly into anomaly detection, using real-world data validation and a rolling window analysis for real-time monitoring. This enhances the adaptability and robustness of LLMs in dynamic CPS environments, enabling quick detection of new anomalies.
Overall, these advancements demonstrate the significant impact of LLMs in enhancing anomaly detection across diverse domains by improving accuracy, scalability, and explanatory power.



\begin{comment}
The application of Large Language Models (LLMs) in anomaly detection within Cyber-Physical Systems (CPS) has gained significant attention due to the potential of these models to enhance system resilience and adaptability. LLMs, such as GPT-4, have demonstrated remarkable capabilities in processing and understanding vast amounts of data, making them suitable for tasks involving anomaly detection where traditional methods might fall short.
A comprehensive framework was introduced for assuring LLM-enabled CPS, focusing on the challenges and risks associated with integrating LLMs into these systems \cite{b15}. The framework addresses critical issues such as context grounding, safety and temporal requirements, and formal verification, ensuring that LLMs can be reliably deployed in CPS for tasks like anomaly detection. This approach is crucial for maintaining system integrity when using probabilistic models like LLMs in environments that demand deterministic behavior.
The concept of "Penetrative AI" was proposed to explore how LLMs can comprehend and interact with the physical world through IoT sensors and actuators \cite{b16}. It was demonstrated that LLMs, when equipped with embedded world knowledge, can effectively interpret IoT sensor data and perform anomaly detection tasks in CPS. This method shows promise for extending the capabilities of LLMs beyond text-based tasks, enabling their use in real-time monitoring and anomaly detection in complex environments.
Another study investigated the use of LLMs for analyzing sensor data in CPS, particularly focusing on the interpretation of data streams from smart devices \cite{b17}. The research highlighted the potential of LLMs to identify anomalous patterns by understanding the context and expected behavior of physical systems, thus enhancing the accuracy and reliability of anomaly detection processes.
In a related study, the integration of LLMs with Programmable Logic Controllers (PLCs) in industrial CPS was explored \cite{b18}. An LLM-based system was developed to assist in monitoring and diagnosing anomalies in industrial processes by analyzing control logic and sensor outputs. This approach is particularly beneficial in environments where real-time decision-making and quick response to anomalies are critical.
Further discussion focused on the challenges and opportunities of using LLMs in CPS, emphasizing the need for robust assurance frameworks to mitigate risks associated with LLM deployment \cite{b19}. The importance of formal verification and context-aware modeling was underscored in ensuring that LLM-based systems can safely and effectively detect anomalies in CPS.
A systematic literature review provided a comprehensive examination of the application of LLMs in forecasting and anomaly detection, highlighting both the current state of research and the challenges ahead \cite{b20}. The review identified critical challenges such as the reliance on vast historical datasets, issues with generalizability across different contexts, and the substantial computational resources required for LLM deployment. The insights offered in this work are valuable for optimizing and applying LLMs to anomaly detection in CPS, particularly in scenarios where traditional methods may struggle to maintain accuracy and efficiency.
Overall, the use of LLMs for anomaly detection in CPS represents a promising area of research, with the potential to significantly enhance system monitoring and fault detection capabilities. As LLMs continue to evolve, their integration into CPS will likely become more widespread, offering new possibilities for improving the safety, reliability, and efficiency of these critical systems.


\subsection{Our Approach}
While the existing methods demonstrate significant advancements in anomaly detection, particularly through the integration of Large Language Models (LLMs) and physical invariants, they still face challenges in scalability, generalization, and the ease of deployment across diverse Cyber-Physical Systems (CPS). Traditional approaches often require extensive domain-specific knowledge to define and extract physical invariants, making them less scalable and more difficult to apply across different CPS architectures. Moreover, while LLMs have been successfully employed to automate some of these processes, the risk of model hallucination and the challenge of effectively validating inferred invariants remain significant obstacles.
Our approach addresses these limitations by proposing a novel method that leverages the capabilities of state-of-the-art LLMs not only to infer physical invariants from CPS documentation but also to validate these invariants using a systematic multi-phase process. The primary motivation behind our method is to enhance the scalability and robustness of anomaly detection in CPS by reducing the dependency on domain expertise and minimizing the risk of false positives due to incorrect invariant inference.
Our method, termed \textit{AnomalyLLM}, is designed to automatically extract potential physical invariants from CPS documentation using LLM-powered intelligent agents. These agents parse the documentation, identify key components and their relationships, and generate hypothetical physical invariants. These invariants are then validated against real-world data through a rigorous cross-validation process to ensure their accuracy and applicability. By integrating validated physical invariants into the anomaly detection framework, our method improves the detection of subtle anomalies that might be overlooked by other approaches.
\end{comment}







\begin{comment}
% Video


Recent advancements in anomaly detection, particularly within Cyber-Physical Systems (CPS) and video surveillance, have increasingly leveraged the capabilities of Large Language Models (LLMs). An innovative approach for Video Anomaly Detection (VAD) using Video-based Large Language Models (VLLMs) has been introduced. Their method, VAD-LLaMA, integrates VLLMs into the VAD framework, enabling the system to detect anomalies in long-range surveillance videos and provide textual explanations for these anomalies, effectively addressing challenges associated with thresholding in traditional anomaly detection methods \cite{b33}. 
Another expansion on the use of LLMs for anomaly detection applies them to CPS. This work focuses on the extraction of physical invariants from system documentation through LLMs, which are then used to identify deviations indicative of anomalies, thereby reducing the labor-intensive nature of manually defining these invariants \cite{b31}. In the context of Industrial Control Systems (ICS), research has explored how LLMs can automate the extraction of operational invariants, crucial for monitoring the normal functioning of ICS. This automation enhances scalability and reduces the dependency on domain-specific knowledge, thus improving the overall efficiency of anomaly detection systems \cite{b32}.
Similarly, investigations into the application of LLMs in smart grids focus on real-time anomaly detection by integrating LLMs with traditional statistical analysis. This hybrid model enhances detection accuracy by considering both historical data and real-time sensor inputs, thereby increasing robustness in dynamic environments \cite{b30}. 
Lastly, challenges of scalability and usability in anomaly detection are addressed by utilizing LLMs to simplify the invariant extraction process, making it more accessible and less reliant on expert knowledge, a significant advancement for large-scale deployments \cite{b34}.

    
\end{comment}






\begin{comment}
% Our Approach
Our approach diverges by utilizing Large Language Models (LLMs) to automatically extract physical invariants from CPS documentation, reducing reliance on domain expertise and improving scalability. This method validates extracted invariants against real-world data, enhancing detection accuracy and identifying subtle anomalies often overlooked by traditional methods. 
While existing LLM-based methods show significant potential, our approach, \textit{AnomalyLLM}, further advances this by integrating LLM-driven invariant extraction into the anomaly detection process. \textit{AnomalyLLM} automates invariant extraction and validates them with real-world data, ensuring reliability. Additionally, it incorporates a rolling window analysis on real-time data streams, enabling prompt and accurate anomaly detection. This enhances the robustness and adaptability of LLMs in dynamic CPS environments, where rapid response to new anomalies is essential.
Collectively, these studies highlight the transformative role of LLMs in improving anomaly detection across various domains, from video surveillance to industrial control systems, by enhancing detection capabilities and providing more comprehensive and explainable results.

\end{comment}









